Uniform Complete Observability of Mass and Rotational Inertial Parameters in Adaptive Identification of Rigid-Body Plant Dynamics

This paper addresses the long-standing open problem of observability of mass and inertia plant parameters in the adaptive identification (AID) of second-order nonlinear models of 6 degree-of-freedom rigid-body dynamical systems subject to externally applied forces and moments. Although stable methods for AID of plant parameters for this class of systems, as well numerous approaches to stable model-based direct adaptive trajectory-tracking control of such systems, have been reported, these studies have been unable to prove analytically that the adaptive parameter estimates converge to the true plant parameter values. This paper reports necessary and sufficient conditions for the uniform complete observability (UCO) of 6-DOF plant inertial parameters for a stable adaptive identifier for this class of systems. When the UCO condition is satisfied, the adaptive parameter estimates are shown to converge to the true plant parameter values. To the best of our knowledge this is the first reported proof for this class of systems of UCO of plant parameters and for convergence of adaptive parameter estimates to true parameter values. We also report a numerical simulation study of this AID approach which shows that (a) the UCO condition can be met for fully-actuated plants as well as underactuated plants with the proper choice of control input and (b) convergence of adaptive parameter estimates to the true parameter values. We conjecture that this approach can be extended to include other parameters that appear rigid body plant models including parameters for drag, buoyancy, added mass, bias, and actuators.

==> acro.tex <==

%\acrodef{6-DOF}{six degree of freedom}
%\acrodef{3-DOF}{three degree of freedom}
%\acrodef{1-DOF}{one degree of freedom}
\acrodef{AI}{adaptive identification} 
\acrodef{DOF}{degree of freedom}
\acrodef{EOM}{equations of motion}
\acrodef{UUV}{unmanned underwater vehicle}
\acrodef{UUVs}{unmanned underwater vehicles}
\acrodef{AID}{adaptive identifier}
\acrodef{RANSAC}{random sample consensus}
\acrodef{DIRANSAC}{Dynamical Plant Identification using RANSAC}
\acrodef{COM}{center of mass}
\acrodef{PDS}{positive definite symmetric}
\acrodef{ML}{machine learning}
\acrodef{NN}{neural net}
\acrodef{ROV}{remotely operated vehicle}
\acrodef{JHU}{Johns Hopkins University}
\acrodef{TLS}{Total Least Squares}
\acrodef{OLS}{Ordinary Least Squares}
\acrodef{NBLS}{Nullspace Based Least Squares}
\acrodef{MAE}{mean absolute error}

\acrodef{MSAC}{M-estimator SAC}
\acrodef{MLESAC}{Maximum Likelihood SAC}
\acrodef{LO-RANSAC}{Locally Optimized RANSAC}
\acrodef{PROSAC}{Progressive SAC}
\acrodef{R-RANSAC}{Randomized RANSAC}
\acrodef{SPRT}{Sequential Probability Ratio Test}
\acrodef{LMedS}{Least Median of Squares}
\acrodef{u-MLESAC}{MLESAC using the estimate of the error variance}
\acrodef{MAPSAC}{Maximum A Posterior Estimation SAC}


==> results.tex <==
\section{Preliminary Simulation Results} 
\label{sec.results} 

\begin{figure}[t]
	\includegraphics[width=0.5\textwidth]{figs/3DOF_Fully_Actuated_With_Noise_CROSS_Final_crop_Scaled.png}
	\vspace*{-7mm}
	\caption{Simulation of fully actuated UUV with CROSS control input}
    \label{fig:3DOFSystemFA_CROSS}
    \vspace{10mm}
  \includegraphics[width=1\linewidth]{figs/3DOF_Under_Actuated_With_Noise_CROSS_Final_crop_Scaled.png}
  	\vspace*{-7mm}
  \caption{Simulation of underactuated UUV with CROSS control input}
  \label{fig:3DOFSystemUA_CROSS}
\end{figure}
Plots of plant velocites for the fully actuated 3-\ac{DOF} \ac{UUV} in the CROSSIM are shown in Figure \ref{fig:3DOFSystemFA_CROSS}, while the corresponding plots of the underactuated 3-\ac{DOF} \ac{UUV} are shown in Figure \ref{fig:3DOFSystemUA_CROSS}.  The forward simulation with the ``true'' parameter values is noted as ``V True'', the simulation using the parameters identified using \ac{OLS} is noted as ``V OLS'' and the simulation using the adaptively identified parameters is noted as ``V AD''.  The trace noted as ``V Init'' shows the plant velocities of a simulated plant using the parameters as initialized in the \ac{AID} algorithm.  All figures show just over 200 seconds of a 2000 second simulation.

The \ac{MAE} for all simulation studies are summarized in Table \ref{tab:MAE_all}.

\begin{table*}
\begin{center}
  \centering
  \caption{Mean Absolute Error of Simulated, 3-DOF UUV Plant Using Identified Parameters with CROSS control input}
  \label{tab:MAE_all}
  \begin{tabular}{ ccllll}
          &  	    & Fully Actuated   & Fully Actuated	&  Under Actuated   & Under Actuated   \\
    DOF   & Simulation	    & AD ID Plant      & LS ID Plant     &  AD ID Plant      & LS ID Plant      \\ \hline
    $v_1$ & IDSIM   & 0.0163 $m/s$     &  0.0845 $m/s$   &  0.0160 $m/s$     &  0.0620 $m/s$    \\  
    $v_1$ & CROSSIM & 0.0203 $m/s$     &  0.0944 $m/s$   &  0.0163 $m/s$     &  0.0596 $m/s$    \\ 
    $v_2$ & IDSIM   & 0.0144 $m/s$     &  0.0748 $m/s$   &  0.0119 $m/s$     &  0.0532 $m/s$    \\  
    $v_2$ & CROSSIM & 0.0201 $m/s$     &  0.0821 $m/s$   &  0.0133 $m/s$     &  0.0423 $m/s$    \\ 
    $v_6$ & IDSIM   & 0.0097 $rad/s$   &  0.0597 $rad/s$ &  0.0113 $rad/s$   &  0.0431 $rad/s$  \\ 
    $v_6$ & CROSSIM & 0.0120 $rad/s$   &  0.0483 $rad/s$ &  0.0121 $rad/s$   &  0.0335 $rad/s$  
  \end{tabular}
  \end{center}
\end{table*}
